On the Applicability of Language Models to Block-Based Programs

Block-based programming languages like Scratch are increasingly popular for programming education and end-user programming. Recent program analyses build on the insight that source code can be modelled using techniques from natural language processing. Many of the regularities of source code that support this approach are due to the syntactic overhead imposed by textual programming languages. This syntactic overhead, however, is precisely what block-based languages remove in order to simplify programming. Consequently, it is unclear how well this modelling approach performs on block-based programming languages. In this paper, we investigate the applicability of language models for the popular block-based programming language Scratch. We model Scratch programs using n-gram models, the most essential type of language model, and transformers, a popular deep learning model. Evaluation on the example tasks of code completion and bug finding confirm that blocks inhibit predictability, but the use of language models is nevertheless feasible. Our findings serve as foundation for improving tooling and analyses for block-based languages.

==> bugram_macros.tex <==
\newcommand{\pearsonfourfailed_sequence_bug}{0.822\xspace}
\newcommand{\pvaluefourfailed_sequence_bug}{0.004\xspace}
\newcommand{\pearsonfourfailed_tests_discovered}{0.902\xspace}
\newcommand{\pvaluefourfailed_tests_discovered}{<0.001\xspace}
\newcommand{\pearsonrandom_fourfailed_sequence_bug}{0.575\xspace}
\newcommand{\pvaluerandom_fourfailed_sequence_bug}{0.082\xspace}
\newcommand{\pearsonrandom_fourfailed_tests_discovered}{0.851\xspace}
\newcommand{\pvaluerandom_fourfailed_tests_discovered}{0.002\xspace}
\newcommand{\pearsonfourfailed_sequence_bug}{0.822\xspace}
\newcommand{\pvaluefourfailed_sequence_bug}{0.004\xspace}
\newcommand{\pearsonfourfailed_tests_discovered}{0.902\xspace}
\newcommand{\pvaluefourfailed_tests_discovered}{<0.001\xspace}
\newcommand{\pearsonrandom_fourfailed_sequence_bug}{0.575\xspace}
\newcommand{\pvaluerandom_fourfailed_sequence_bug}{0.082\xspace}
\newcommand{\pearsonrandom_fourfailed_tests_discovered}{0.851\xspace}
\newcommand{\pvaluerandom_fourfailed_tests_discovered}{0.002\xspace}


==> img/bugram_example.tex <==
\begin{scratch}
\setscratch{scale=0.88}
\blockinit{When \greenflag clicked}
\blocklook{set size to \ovalnum{50} \%}
\blockmove{go to x: \ovaloperator{pick random \ovalnum{230} to \ovalnum{-230}}
                 y: \ovalnum{170}}
\blockinfloop{forever}
{
\blockmove{change y by \ovalnum{-7}}
\blockif{if \boolsensing{touching color \pencolor{red} ?} then}
{
\blocklook{say \ovalnum{-8} for \ovalnum{1} seconds}
\blockvariable{change \selectmenu{points} by \ovalnum{-8}}
\blockmove{go to x: \ovaloperator{pick random \ovalnum{230} to \ovalnum{-230}}
                 y: \ovalnum{170}}
}
\blockif{if \boolsensing{touching \selectmenu{Bowl} ?} then}
{
\blockvariable{change \selectmenu{points} by \ovalnum{8}}
\blockmove{go to x: \ovaloperator{pick random \ovalnum{230} to \ovalnum{-230}}
                 y: \ovalnum{170}}
}
}
\end{scratch}
\setscratch{scale=0.55}

==> tables/bugram_random_bottom_intersection_table.tex <==
\begin{table}
\centering
\caption{Percentage of how much sequences the bottom and random ten sequences had in common}
\label{tab:bugram_random_bottom_intersection}
\begin{tabular}{lr}
\toprule
{} &  intersection bottom/random (\%) \\
\midrule
K6\_S01 &                              10 \\
K6\_S12 &                              10 \\
K6\_S15 &                              10 \\
K6\_S18 &                              20 \\
K6\_S31 &                              10 \\
K7\_S03 &                              30 \\
K7\_S10 &                              20 \\
K7\_S14 &                              20 \\
K7\_S17 &                              10 \\
K7\_S24 &                              20 \\
\midrule
Sum    &                              16 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bugram_sequence3_table.tex <==
\begin{table}
\centering
\caption{Number of code sequences of length 3 containing at least one bug, number of found bugs and bugs in total as well as the percentage of found bugs.}
\label{tab:bugram_sequence_table3}
\begin{tabular}{lrrrr}
\toprule
& \begin{tabular}[c]{@{}l@{}}\#bugs\\ found\end{tabular} & \begin{tabular}[c]{@{}l@{}}\#bugs\\ in total\end{tabular}  & P@10 & \begin{tabular}[c]{@{}l@{}}bugs\\ found (\%) \end{tabular} \\ 
\midrule
K6\_S01  &         26.0 &            27.0 &  1.00 &           96.30 \\
K6\_S12  &         21.0 &            26.0 &  0.60 &           80.77 \\
K6\_S15  &          7.0 &            16.0 &  0.50 &           43.75 \\
K6\_S18  &          2.0 &             6.0 &  0.40 &           33.33 \\
K6\_S31  &          1.0 &             8.0 &  0.10 &           12.50 \\
K7\_S03  &         10.0 &            11.0 &  0.70 &           90.91 \\
K7\_S10  &          1.0 &             7.0 &  0.10 &           14.29 \\
K7\_S14  &          3.0 &             5.0 &  0.30 &           60.00 \\
K7\_S17  &          2.0 &             2.0 &  0.20 &          100.00 \\
K7\_S24  &          3.0 &            24.0 &  0.60 &           12.50 \\
\midrule
Average &          7.6 &            13.2 &  0.45 &           57.58 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bugram_sequence4_table.tex <==
\begin{table}
\centering
\caption{Number of code sequences of length 4 containing at least one bug, number of found bugs and bugs in total as well as the percentage of found bugs.}
\label{tab:bugram_sequence_table4}
\begin{tabular}{lrrrr}
\toprule
& \begin{tabular}[c]{@{}l@{}}\#bugs\\ found\end{tabular} & \begin{tabular}[c]{@{}l@{}}\#bugs\\ in total\end{tabular}  & P@10 & \begin{tabular}[c]{@{}l@{}}bugs\\ found (\%) \end{tabular} \\ 
\midrule
K6\_S01  &         26.0 &            27.0 &  0.90 &           96.30 \\
K6\_S12  &         21.0 &            26.0 &  0.60 &           80.77 \\
K6\_S15  &         10.0 &            16.0 &  0.60 &           62.50 \\
K6\_S18  &          3.0 &             6.0 &  0.60 &           50.00 \\
K6\_S31  &          6.0 &             8.0 &  0.30 &           75.00 \\
K7\_S03  &          3.0 &            11.0 &  0.60 &           27.27 \\
K7\_S10  &          2.0 &             7.0 &  0.20 &           28.57 \\
K7\_S14  &          3.0 &             5.0 &  0.30 &           60.00 \\
K7\_S17  &          1.0 &             2.0 &  0.10 &           50.00 \\
K7\_S24  &          8.0 &            24.0 &  0.70 &           33.33 \\
\midrule
Average &          8.3 &            13.2 &  0.49 &           62.88 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bugram_sequence5_table.tex <==
\begin{table}
\centering
\caption{Number of code sequences of length 5 containing at least one bug, number of found bugs and bugs in total as well as the percentage of found bugs.}
\label{tab:bugram_sequence_table5}
\begin{tabular}{lrrrr}
\toprule
& \begin{tabular}[c]{@{}l@{}}\#bugs\\ found\end{tabular} & \begin{tabular}[c]{@{}l@{}}\#bugs\\ in total\end{tabular}  & P@10 & \begin{tabular}[c]{@{}l@{}}bugs\\ found (\%) \end{tabular} \\ 
\midrule
K6\_S01  &         26.0 &            27.0 &  0.90 &           96.30 \\
K6\_S12  &         21.0 &            26.0 &  0.60 &           80.77 \\
K6\_S15  &          7.0 &            16.0 &  0.70 &           43.75 \\
K6\_S18  &          3.0 &             6.0 &  0.80 &           50.00 \\
K6\_S31  &          6.0 &             8.0 &  0.40 &           75.00 \\
K7\_S03  &         10.0 &            11.0 &  0.70 &           90.91 \\
K7\_S10  &          1.0 &             7.0 &  0.20 &           14.29 \\
K7\_S14  &          2.0 &             5.0 &  0.30 &           40.00 \\
K7\_S17  &          1.0 &             2.0 &  0.10 &           50.00 \\
K7\_S24  &          8.0 &            24.0 &  0.80 &           33.33 \\
\midrule
Average &          8.5 &            13.2 &  0.55 &           64.39 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bugram_sequence6_table.tex <==
\begin{table}
\centering
\caption{Number of code sequences of length 6 containing at least one bug, number of found bugs and bugs in total as well as the percentage of found bugs.}
\label{tab:bugram_sequence_table6}
\begin{tabular}{lrrrr}
\toprule
& \begin{tabular}[c]{@{}l@{}}\#bugs\\ found\end{tabular} & \begin{tabular}[c]{@{}l@{}}\#bugs\\ in total\end{tabular}  & P@10 & \begin{tabular}[c]{@{}l@{}}bugs\\ found (\%) \end{tabular} \\ 
\midrule
K6\_S01  &         26.0 &            27.0 &   0.9 &           96.30 \\
K6\_S12  &         21.0 &            26.0 &   0.6 &           80.77 \\
K6\_S15  &          6.0 &            16.0 &   0.8 &           37.50 \\
K6\_S18  &          2.0 &             6.0 &   0.8 &           33.33 \\
K6\_S31  &          1.0 &             8.0 &   0.4 &           12.50 \\
K7\_S03  &          5.0 &            11.0 &   0.7 &           45.45 \\
K7\_S10  &          3.0 &             7.0 &   0.3 &           42.86 \\
K7\_S14  &          2.0 &             5.0 &   0.5 &           40.00 \\
K7\_S17  &          1.0 &             2.0 &   0.1 &           50.00 \\
K7\_S24  &          7.0 &            24.0 &   0.9 &           29.17 \\
\midrule
Average &          7.4 &            13.2 &   0.6 &           56.06 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/bugram_sequencerandom_4_table.tex <==
\begin{table}
\centering
\caption{Number of code sequences of length random 4 containing at least one bug, number of found bugs and bugs in total as well as the percentage of found bugs.}
\label{tab:bugram_sequence_tablerandom_4}
\begin{tabular}{lrrrr}
\toprule
& \begin{tabular}[c]{@{}l@{}}\#bugs\\ found\end{tabular} & \begin{tabular}[c]{@{}l@{}}\#bugs\\ in total\end{tabular}  & P@10 & \begin{tabular}[c]{@{}l@{}}bugs\\ found (\%) \end{tabular} \\ 
\midrule
K6\_S01  &         10.0 &            27.0 &  0.40 &           37.04 \\
K6\_S12  &          7.0 &            26.0 &  0.90 &           26.92 \\
K6\_S15  &          5.0 &            16.0 &  0.30 &           31.25 \\
K6\_S18  &          3.0 &             6.0 &  0.50 &           50.00 \\
K6\_S31  &          1.0 &             8.0 &  0.10 &           12.50 \\
K7\_S03  &          5.0 &            11.0 &  0.40 &           45.45 \\
K7\_S10  &          0.0 &             7.0 &  0.00 &            0.00 \\
K7\_S14  &          1.0 &             5.0 &  0.20 &           20.00 \\
K7\_S17  &          1.0 &             2.0 &  0.10 &           50.00 \\
K7\_S24  &          5.0 &            24.0 &  0.50 &           20.83 \\
\midrule
Average &          3.8 &            13.2 &  0.34 &           28.79 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/metrics.tex <==
\begin{table}
\centering
\caption{Average metrics for the training and evaluation dataset.}
\label{tab:metrics}
\begin{tabular}{lrrrr}
\toprule
{} &  training &  evaluation \\
\midrule
\#blocks               &     89.93 &       87.99 \\
Length Longest Script &     15.41 &       15.30 \\
Weighted Method Count &     22.80 &       22.54 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics_100k.tex <==
\begin{table}
\centering
\caption{Average metrics for the 100,000 projects in the training set.}
\label{tab:metrics_100k}
\begin{tabular}{lr}
\toprule
\#blocks               &  89.93 \\
Length Longest Script &  15.41 \\
Weighted Method Count &  22.80 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics_100k_transposed.tex <==
\begin{table}
\centering
\caption{Average metrics for the 100,000 projects in the training set.}
\label{tab:metrics_100k}
\begin{tabular}{rrrrrrrrrr}
\toprule
 \#blocks &  Length Longest Script &  Weighted Method Count \\
\midrule
   89.93 &                  15.41 &                   22.8 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics_10k.tex <==
\begin{table}
\centering
\caption{Average metrics for the 10,000 projects used for evaluation.}
\label{tab:metrics_10k}
\begin{tabular}{lr}
\toprule
\#blocks               &  87.99 \\
Length Longest Script &  15.30 \\
Weighted Method Count &  22.54 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics_10k_transposed.tex <==
\begin{table}
\centering
\caption{Average metrics for the 10,000 projects used for evaluation.}
\label{tab:metrics_10k}
\begin{tabular}{rrrrrrrrrr}
\toprule
 \#blocks &  Length Longest Script &  Weighted Method Count \\
\midrule
   87.99 &                   15.3 &                  22.54 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/metrics_transposed.tex <==
\begin{table}
\centering
\caption{Average metrics for the training and evaluation dataset.}
\label{tab:metrics}
\begin{tabular}{rrr}
\toprule
 \#blocks &  Length Longest Script &  Weighted Method Count \\
\midrule
   89.93 &                  15.41 &                  22.80 \\
   87.99 &                  15.30 &                  22.54 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/top_recall.tex <==
\begin{table}[]
\caption{Best predicted blocks in terms of recall}
\label{tab:completion-top-recall}
\begin{tabular}{lrrr}
\toprule
Block & Occurrence & Usage-Rank & Recall   \\
\midrule
\begin{scratch}\blockinit{When \greenflag clicked}\end{scratch} & \SI[round-mode=places, round-precision=2]{6.053139379545792}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{95.69641981363414}{\percent}\\
\booloperator{\ovalnum{} = \ovalnum{}} & \SI[round-mode=places, round-precision=2]{2.8279154915639997}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{95.48158516315284}{\percent}\\
\boolsensing{touching \selectmenu{} ?} & \SI[round-mode=places, round-precision=2]{1.8896887833358071}{\percent} & \num[round-mode=places, round-precision=0]{4.0} & \SI[round-mode=places, round-precision=2]{90.835897100216}{\percent}\\
\ovalvariable{var} & \SI[round-mode=places, round-precision=2]{4.896343575280788}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{90.54415925626516}{\percent}\\
\boolsensing{key \selectmenu{} pressed ?} & \SI[round-mode=places, round-precision=2]{1.195141259710059}{\percent} & \num[round-mode=places, round-precision=0]{5.0} & \SI[round-mode=places, round-precision=2]{83.92672324570482}{\percent}\\
\bottomrule
\end{tabular}
\end{table}


==> tables/top_recall_all.tex <==
\begin{table}[]
\caption{Top two best predicted blocks for each category in terms of top-3 accuracy}\label{tab:completion-top-recall}
\begin{tabular}{lrrr}
\toprule
Block & Occurrence & \begin{tabular}[c]{@{}l@{}}Occurrence-Rank\\ in Category \end{tabular} & \begin{tabular}[c]{@{}l@{}}Top-3\\ Accuracy \end{tabular}   \\
\midrule
\begin{scratch}\blockinfloop{forever}{\blockspace[0.5]}\end{scratch} & \SI[round-mode=places, round-precision=2]{3.8901587739478702}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{73.39728369265838}{\percent}\\
\begin{scratch}\blockcontrol{wait \ovalnum{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{6.244796618602612}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{72.46282491223918}{\percent}\\
\ovalvariable{var} & \SI[round-mode=places, round-precision=2]{4.901031070036898}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{90.81040331699963}{\percent}\\
\begin{scratch}\blocklist{add \ovalnum{} to \selectmenu{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.2495159931623258}{\percent} & \num[round-mode=places, round-precision=0]{6.0} & \SI[round-mode=places, round-precision=2]{68.31194471865746}{\percent}\\
\begin{scratch}\blockinit{when \greenflag clicked}\end{scratch} & \SI[round-mode=places, round-precision=2]{6.0268088062149925}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{95.51659310119341}{\percent}\\
\begin{scratch}\blockevent{broadcast \ovalcontrol*{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{1.962136625400876}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{40.96786341953301}{\percent}\\
\ovallook{costume \selectmenu{}} & \SI[round-mode=places, round-precision=2]{0.2854778243584754}{\percent} & \num[round-mode=places, round-precision=0]{13.0} & \SI[round-mode=places, round-precision=2]{79.98274374460742}{\percent}\\
\begin{scratch}\blocklook{hide}\end{scratch} & \SI[round-mode=places, round-precision=2]{4.293990433167647}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{77.07508747777204}{\percent}\\
\ovalmove{y position} & \SI[round-mode=places, round-precision=2]{0.28707886478844097}{\percent} & \num[round-mode=places, round-precision=0]{12.0} & \SI[round-mode=places, round-precision=2]{77.69197769197768}{\percent}\\
\ovalmove{x position} & \SI[round-mode=places, round-precision=2]{0.3050597803865158}{\percent} & \num[round-mode=places, round-precision=0]{10.0} & \SI[round-mode=places, round-precision=2]{70.04440855874041}{\percent}\\
\booloperator{\ovalnum{} = \ovalnum{}} & \SI[round-mode=places, round-precision=2]{2.8175848428270927}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{95.4716321356762}{\percent}\\
\ovaloperator{letter \ovalnum{} to \ovalnum{}} & \SI[round-mode=places, round-precision=2]{0.22106673629139922}{\percent} & \num[round-mode=places, round-precision=0]{13.0} & \SI[round-mode=places, round-precision=2]{71.36490250696379}{\percent}\\
\begin{scratch}\blockpen{pen up}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.19077012507820468}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{51.452550032278886}{\percent}\\
\begin{scratch}\blockpen{set pen size to \ovalnum{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.09249087406954919}{\percent} & \num[round-mode=places, round-precision=0]{5.0} & \SI[round-mode=places, round-precision=2]{47.27030625832223}{\percent}\\
\boolsensing{touching \selectmenu{} ?} & \SI[round-mode=places, round-precision=2]{1.881715133034144}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{90.85018653053211}{\percent}\\
\boolsensing{key \selectmenu{} pressed ?} & \SI[round-mode=places, round-precision=2]{1.1967161429211846}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{84.49109807553772}{\percent}\\
\begin{scratch}\blocksound{play sound \ovalsound*{} until done}\end{scratch} & \SI[round-mode=places, round-precision=2]{1.233786386722695}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{44.689558794170495}{\percent}\\
\begin{scratch}\blocksound{change \selectmenu{} effect by \ovalnum{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.015271462562748469}{\percent} & \num[round-mode=places, round-precision=0]{7.0} & \SI[round-mode=places, round-precision=2]{38.70967741935484}{\percent}\\
\begin{scratch}\blockmoreblocks{call}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.9352539250121925}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{41.32209639188833}{\percent}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/top_recall_shape.tex <==
\begin{table}[]
\caption{Top two best predicted blocks for each shape in terms of top-3 accuracy}\label{tab:completion-top-recall-shape}
\begin{tabular}{lrrr}
\toprule
Block & Occurrence & \begin{tabular}[c]{@{}l@{}}Occurrence-Rank\\ in shape \end{tabular} & \begin{tabular}[c]{@{}l@{}}Top-3\\ Accuracy \end{tabular}     \\
\midrule
\ovalvariable{var} & \SI[round-mode=places, round-precision=2]{4.901031070036898}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{90.81040331699963}{\percent}\\
\ovalsensing{answer} & \SI[round-mode=places, round-precision=2]{0.5479252979166769}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{83.59181838615419}{\percent}\\
\begin{scratch}\blocklook{hide}\end{scratch} & \SI[round-mode=places, round-precision=2]{4.293990433167647}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{77.07508747777204}{\percent}\\
\begin{scratch}\blockcontrol{wait \ovalnum{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{6.244796618602612}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{72.46282491223918}{\percent}\\
\begin{scratch}\blockinfloop{forever}{\blockspace[0.5]}\end{scratch} & \SI[round-mode=places, round-precision=2]{3.8901587739478702}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{73.39728369265838}{\percent}\\
\begin{scratch}\blockif{if \boolempty[2em] then}{\blockspace[0.5]}\end{scratch} & \SI[round-mode=places, round-precision=2]{4.4088958732567125}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{71.95452386938183}{\percent}\\
\begin{scratch}\blockstop{delete this clone}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.423167301335514}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{30.67520372526193}{\percent}\\
\begin{scratch}\blockstop{stop \selectmenu{}}\end{scratch} & \SI[round-mode=places, round-precision=2]{0.8266294896868365}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{29.499404052443378}{\percent}\\
\booloperator{\ovalnum{} = \ovalnum{}} & \SI[round-mode=places, round-precision=2]{2.8175848428270927}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{95.4716321356762}{\percent}\\
\boolsensing{touching \selectmenu{} ?} & \SI[round-mode=places, round-precision=2]{1.881715133034144}{\percent} & \num[round-mode=places, round-precision=0]{2.0} & \SI[round-mode=places, round-precision=2]{90.85018653053211}{\percent}\\
\begin{scratch}\blockinit{when \greenflag clicked}\end{scratch} & \SI[round-mode=places, round-precision=2]{6.0268088062149925}{\percent} & \num[round-mode=places, round-precision=0]{1.0} & \SI[round-mode=places, round-precision=2]{95.51659310119341}{\percent}\\
\begin{scratch}\blockinit{when \selectmenu{} key pressed}\end{scratch} & \SI[round-mode=places, round-precision=2]{1.3259077899237903}{\percent} & \num[round-mode=places, round-precision=0]{3.0} & \SI[round-mode=places, round-precision=2]{20.66691436002229}{\percent}\\
\bottomrule
\end{tabular}
\end{table}
